Scaling up HBM Efficiency of Top-K SpMV for Approximate Embedding Similarity on FPGAs

Top-K SpMV is a key component of similarity-search on sparse embeddings. This sparse workload does not perform well on general-purpose NUMA systems that employ traditional caching strategies. Instead, modern FPGA accelerator cards have a few tricks up their sleeve. We introduce a Top-K SpMV FPGA design that leverages reduced precision and a novel packet-wise CSR matrix compression, enabling custom data layouts and delivering bandwidth efficiency often unreachable even in architectures with higher peak bandwidth. With HBM-based boards, we are 100x faster than a multi-threaded CPU implementation and 2x faster than a GPU with 20% higher bandwidth, with 14.2x higher power-efficiency.

==> code/ppr.tex <==
\begin{algorithm}
  \caption{Personalized PageRank}\label{alg:ppr}
  \begin{algorithmic}[1]
    \Function{PPR}{$coo\_graph, \mathbf{\bar{V}}, \mathbf{\bar{d}}, \alpha, max\_iter$}
      \State Initialize local buffers to $0$
      \For{$k \gets 0,\kappa$} \Comment{Set PR=1 on pers. vertices}
        \State $\mathbf{P_1}[k] = \mathbf{\bar{V}}[k]$
      \EndFor
      \For{$i \gets 0,max\_iter$} 
        \State $scaling\_vec \gets scaling(\mathbf{P_1},\mathbf{\bar{d}})$ \Comment{$i.e.\ \frac{\alpha}{|V|}\mathbf{P_1}\mathbf{\bar{d}}$}
        
        \State $SpMV(coo\_graph, \mathbf{P_1}, \mathbf{P_2})$ \Comment{$\mathbf{Xp_i}$ in \cref{eq:ppr}}
        \State $\mathbf{P_1} = \alpha \mathbf{P_2} + scaling\_vec + (1-\alpha)\mathbf{\bar{V}}$
        
      \EndFor
      \State Write $\mathbf{P_1}$ to output
    \EndFunction
  \end{algorithmic}
\end{algorithm}

==> code/scaling.tex <==
\begin{algorithm}
    \caption{Computing the scaling vector of \gls{ppr}}\label{alg:scaling}
    \begin{algorithmic}[1]
    \Function{Scaling}{$\mathbf{P}, \mathbf{\bar{d}}$}
        \LineComment{Blocks have $B$ elements and size $P\_SIZE$}
        \For{$i \gets 0, |V| / B$} 
            \State $dangling = \mathbf{\bar{d}}[i / (P\_SIZE / B)]$
        
            \For{$k \gets 0,\kappa$} 
                \For{$b \gets 0,B$} 
                    \State $d\_buffer[k, b] =$\par
                    \hskip\algorithmicindent$\mathbf{P}[k, i \cdot B + b] + dangling[(i \cdot B + j)\ \%\ P\_SIZE]$
                \EndFor
                \State $dangling\_vals[k, :] \pluseq sum(d\_buffer[k, :])$
            \EndFor
        \EndFor
        \State Return $\alpha \cdot dangling\_vals$
    \EndFunction
    \end{algorithmic}
\end{algorithm}

==> tables/matrices.tex <==
\renewcommand\theadalign{tl}
\renewcommand\theadfont{\bfseries}
% \setlength\tabcolsep{5pt}
% \renewcommand\theadgape{\Gape[10pt]}
% \renewcommand\cellgape{\Gape[10pt]}

\begin{table}
\centering
% \ra{1.2}
    \caption{Matrices used in the evaluation. Every matrix has 512 columns, and rows have 10 to 40 non-zero entries. We report the memory occupation of each matrix on HBM \textcolor{red}{metti nuove matrici}}
    % \resizebox{1\columnwidth}{!}{
	\begin{tabular}{@{}llll@{}}
		\toprule
		\thead{Rows} & \thead{Non-zeros} & \thead{Non-zeros per row} & \thead{Size (MB)} \\
		\midrule
	%	\textbf{$10^4$} & $249\,181$ & $24.91$     & $\SI{2.99}{\mega\byte}$ \\
		\textbf{$10^5$} & $2\,501\,695$ & $25.0$    & $\SI{30.02}{\mega\byte}$ \\
		\textbf{$10^6$} & $25\,001\,784$ & $25.00$  & $\SI{300.02}{\mega\byte}$ \\
		\textbf{$10^7$} & $249\,960\,781$ & $24.99$ & $\SI{3.00}{\giga\byte}$ \\
		\bottomrule
	\end{tabular}
    % }
    \label{tab:matrices}
\end{table}


==> tables/resources.tex <==
\renewcommand\theadalign{tl}
\renewcommand\theadfont{\bfseries}
\setlength\tabcolsep{3pt}
% \renewcommand\theadgape{\Gape[10pt]}
% \renewcommand\cellgape{\Gape[10pt]}

\begin{table}
\centering
\ra{1.0}
    \caption{Resource usage, clock frequency and power consumption of our architecture. Highest values in bold.
    % Floating point arithmetic greatly increases the use of DSPs and LUTs, while LUT utilization and clock frequency change linearly w.r.t bit-width.
    % Other bit-widths, omitted for brevity, show the same trends
    }
    \resizebox{1\linewidth}{!}{
	\begin{tabular}{@{}lllllllll@{}}
		\toprule
	% 2 Lines
% 	& \multirow{2}{*}{\thead{Bit-width}} & \multirow{2}{*}{\thead{BRAM}} & \multirow{2}{*}{\thead{DSP}} & \multirow{2}{*}{\thead{FF}} & \multirow{2}{*}{\thead{LUT}}  & \multirow{2}{*}{\thead{URAM}} &\multirow{2}{*}{\thead{Clock}} & \thead{Power\\Consumption}\\
    % 1 Line
	\multirow{2}{*}{\thead{Bit-width}} & \multirow{2}{*}{\thead{Cores}} & \multirow{2}{*}{\thead{LUT}} & \multirow{2}{*}{\thead{FF}} & \multirow{2}{*}{\thead{BRAM}} & \multirow{2}{*}{\thead{URAM}}  & \multirow{2}{*}{\thead{DSP}} & \thead{Clock\\(MHz)} & \thead{Power\\Cons.}\\
	   
	    \midrule
    	% \textbf{Total resources} &  & 4320 & 6840 & 2364480 & 1182240 & 960 &  &  \\
    	
% 	    100K buffer
    	
		\multirow{2}{*}{\textbf{20 bits}} & 16 & 18\% & 16\% & 26\% & 8\% & 2\% & 362 & 34 W \\
		& \textbf{32} & 38\% & \textbf{34\%} & \textbf{53\%} & \textbf{17\%} & 5\% & 326 & 34 W \\
% 		& 1 & 1\% & 0.6\% & 0.8\% & 0.5\% & 0.1\% &  & \\
		 \midrule
		\multirow{2}{*}{\textbf{24 bits}} & 16 & 19\% & 17\% & 26\% & 8\% & 3\% & \textbf{374} & 35 W \\
		& 28 & 35\% & 30\% & 45\% & 15\% & 6\% & 351 & 35 W \\
% 		& 1 & 1.2\% & 0.7\% & 1.2\% & 0.5\% & 0.2\% & \\
		\midrule
		\multirow{2}{*}{\textbf{32 bits}} & 16 & 21\% & 19\% & 27\% & 8\% & 5\% & 351 & 35 W \\
		& 26 & 36\% & 32\% & 44\% & 14\% & 8\% & 322 & 35 W \\
% 		& 1 & 1.3\% & 0.8\% & 1.2\% & 0.5\% & 0.3\% &  &  \\
    		\midrule
		\textbf{32 bits, float} & 21 & \textbf{43\%} & 28\% & 23\% & 11\% & \textbf{10\%} & 312 & \textbf{45 W} \\
% 		& 1 & 2\% & 1.3\% & 1.1\% & 0.5\% & 0.4\% &  & \\
        \midrule
        \textbf{Available} &  & 1097419 & 2180971 & 1812 & 960 & 9020 & & \\
		\bottomrule
	\end{tabular}
    }
    \label{tab:resources}
\end{table}

==> tables/simul.tex <==
\renewcommand\theadalign{tl}
\renewcommand\theadfont{\bfseries}
\setlength\tabcolsep{3pt}
% \renewcommand\theadgape{\Gape[10pt]}
% \renewcommand\cellgape{\Gape[10pt]}

\begin{table}
\centering
\ra{1.0}
    \caption{Estimation of missing Top-K values for increasing number of partitions. Results are averaged over 30 tests.
    }
    \resizebox{1\linewidth}{!}{
	\begin{tabular}{@{}rcrccrrrrrr@{}}
		\toprule
        
        \thead{Rows} & \thead{Cores} & \phantom{abc} & &
         \multicolumn{6}{c}{\thead{Top-K Value}}\\
        \cmidrule{4-9} & &
        & $\mathbf{8}$ & $\mathbf{16}$ & $\mathbf{32}$ & $\mathbf{50}$ & $\mathbf{75}$ & $\mathbf{100}$\\
        \midrule
        $10^6$ & 21  & 1 & 1 & 1 & 1 & 1 & 1\\
        & 26 &  & 1 & 1 & 1 & 1 & 1 & 1\\
        & 28 & & 1 & 1 & 1 & 1 & 1 & 1\\
        & 32 & & 1 & 1 & 1 & 1 & 1 & 1\\
        $10^7$ & 21 &   & 1 & 1 & 1 & 1 & 1 & 1\\
        & 26 & & 1 & 1 & 1 & 1 & 1 & 1\\
        & 28 & & 1 & 1 & 1 & 1 & 1 & 1\\
        & 32 & & 1 & 1 & 1 & 1 & 1 & 1\\
		\bottomrule 
	\end{tabular}
	}
    \label{tab:error_estimation}
\end{table}

==> tables/simulated.tex <==
\renewcommand\theadalign{tl}
\renewcommand\theadfont{\bfseries}
\setlength\tabcolsep{3pt}
% \renewcommand\theadgape{\Gape[10pt]}
% \renewcommand\cellgape{\Gape[10pt]}

\begin{table}
\centering
\ra{1.0}
    \caption{Top-K SpMV simulated accuracy for different architectures
    % Floating point arithmetic greatly increases the use of DSPs and LUTs, while LUT utilization and clock frequency change linearly w.r.t bit-width.
    % Other bit-widths, omitted for brevity, show the same trends
    }
    \resizebox{1\linewidth}{!}{
	\begin{tabular}{@{}llll@{}}
		\toprule
	\multirow{4}{*}{\thead{Matrix Size}} & \multirow{4}{*}{\thead{Cores}} & \multirow{4}{*}{\thead{Top-K Value}} & \multirow{4}{*}{\thead{Precision}}\\
	   
	    \midrule
		\multirow{4}{*}{\textbf{10^5}} & \multirow{4}{*}{\textbf{21 cores}} & 8 & 1.0 \\
		& & 16 & 1.0 \\
		& & 32 & 1.0 \\
	    & & 100 & 0.986 \\
		\bottomrule
	\end{tabular}
	}
    \label{tab:simulated}
\end{table}
